Understanding the Challenges of Deploying Live-Traceability Solutions

Software traceability is the process of establishing and maintaining relationships between artifacts in a software system. This process is crucial to many engineering processes, particularly for safety critical projects; however, it is labor-intensive and error-prone. Automated traceability has been a long awaited tool for project managers of these systems, and due to the semantic similarities between linked artifacts, NLP techniques, such as transformer models, may be leveraged to accomplish this task. SAFA.ai is a startup focusing on fine-tuning project-specific models that deliver automated traceability in a near real-time environment. The following paper describes the challenges that characterize commercializing software traceability and highlights possible future directions.

==> sections/out_dated/analysis.tex <==
We first chose to analyze three main aspects of the datasets: Flesch Kincaid readability score \cite{kincaid_derivation_1975}, number of out of vocab words, and number of high and low frequency words to see if any of these attributes made the datasets more or less challenging. We also investigate certain attributes of mis-predicted links of three different models across the datasets. 

We do not intend to make any causal claims in this analysis. Instead, we hope to shed light on possible future directions of exploration that might improve model performance on a wider range of datasets.

\subsection{Dataset Analysis}
 The first was the Flesch Kincaid readability score which is based on the word and sentence lengths of the text \cite{kincaid_derivation_1975}. More complex and verbose datasets will achieve a lower readability score, which may also be a factor in model performance. Additionally, we calculated the proportion of low frequency words (i.e. words that make up less than \todo{insert percentage used} of the total dataset) as well as the proportion of high frequency words (i.e. words that make up more than \todo{insert percentage used} of the total dataset). Before making these calculations, we eliminate stop words included in the python package NLTK \cite{nltk}. The motivation for this metric is that many low frequency words, particularly those that intend a non-traditional meaning within the domain context, may be difficult for the model to understand. In contrast, many high frequency words might make artifacts seem more similar to one another than they actually are, resulting in an increase of false positives. Finally, we examine the number of out of vocabulary words for each model, paying particular attention to any acronyms or domain-specific jargon that the model might not be familiar with. To analyze this, we examine the difference between the dataset vocabulary and the vocabulary of the tokenizer for a given model. 

% Ran out of time for this part
% To better understand when a model is struggling to generalize on a dataset, we examine the difference between the train and validation loss of each training run, where a high discrepancy between the losses might be a sign of poor generalization \addcite{}. Additionally, we examined the variability between splits of the data, where we speculated that a greater influence of the splits on model performance could be tied to an increased difficulty of the model to discover relevant patterns in the dataset.

For each run, we further investigated the number of mis-predicted links containing certain qualities that could make them more challenging. Since a high number of overlapping words or many shared synonyms might make the artifacts appear similar despite not actually being linked, we calculated the number of overlapping words between the two artifacts of the mis-predicted links. We also used the NLTK library \cite{nltk} to approximate the number of synonyms and antonyms across the two artifacts. Finally, we calculated the number of misspelled and out of vocabularly words used in both artifacts which could challenge the model's understanding of the text. For this investigation, a a threshold of >=0.5 is used to determine positive links while the rest are considered negative links. This was selected because our training process balances positive and negative classes meaning that 0.5 should be its theoretical threshold under ideal learning circumstances.  % \jch{We need to justify the >=0.5. See OL Comment} 

For the final piece of our analysis, we wanted to discover if all models had similar weaknesses. To gain some insight into this, we measured the number of links that were mis-predicted between two different models on the same dataset split and compared this number to the intersection of mis-predicted links by the same model across different splits of the data. 
\todo{Include the results of the analysis}


% \subsubsection{Results}


==> sections/out_dated/notes.tex <==
% \todo{describe the base approach with RoBERTa \cite{liu_roberta_2019} and the numebr of epochs etc}

% \begin{itemize}
%     \item \cite{Devlin_Chang_Lee_Toutanova_2019} first to publish fine-tuning and made a lot of mistakes.
%     \item Training for 20 epochs and evaluating after each following best practices \cite{Mosbach_Andriushchenko_Klakow_2021}. 
%     \item \cite{Zhang_Wu_Katiyar_Weinberger_Artzi_2021} recommends re-initializing last layers which is similar to freezing initial ones. Recommended epochs of 3 \cite{Devlin_Chang_Lee_Toutanova_2019} is insufficient. 
%     \item \cite{Merchant_Rahimtoroghi_Pavlick_Tenney_2020} shows that "fine-tuning primarily affects the top layers of BERT".
%     \item \cite{Hao_Dong_Wei_Xu_2019} "the lower layers of BERT are more invariant during fine-tuning, which suggests that the layers that are close to input learn more transferable representations of language."
%     \item \cite{sajjad_effect_2023} the lower layers are most critical to maintain downstream task performance, sentence similarity tasks are more robust to the dropping of layers, and models trained using different objective function exhibit different learning patterns and w.r.t the layer dropping
%     \item \cite{tamkin_investigating_2020} earlier layers provide more of an improvement on finetuning performance when the finetuning dataset is large; smaller datasets may leave the network reliant on existing feature processing in those layers. earlier layers appear to be generally more helpful for finetuning relative to the later layers
%     \item \cite{mukherjee_clues_2021} there is a huge gap in performance between humans and modles in the few-shot setting for most tasks
%     \item \cite{wei_eda_2019} considers data augmentation with synonym replacement, random insertion, random swap, and random deletion.
%     \item \cite{von_der_mosel_validity_2022} found that less then half of the commonly used terminology from the general domain is among the commonly used terminology within the SE. this demonstrates that NLP models with a fixed vocabulary should always be retrained from scratch for the SE domain to maximize the performance domain
% \end{itemize}



